FEEBO: An Empirical Evaluation Framework for Malware Behavior Obfuscation

Program obfuscation is increasingly popular among malware creators. Objectively comparing different malware detection approaches with respect to their resilience against obfuscation is challenging. To the best of our knowledge, there is no common empirical framework for evaluating the resilience of malware detection approaches w.r.t. behavior obfuscation. We propose and implement such a framework that obfuscates the observable behavior of malware binaries. To assess the framework's utility, we use it to obfuscate known malware binaries and then investigate the impact on detection effectiveness of different $n$-gram based detection approaches. We find that the obfuscation transformations employed by our framework significantly affect the precision of such detection approaches. Several $n$-gram-based approaches can hence be concluded not to be resilient against this simple kind of obfuscation.

==> parts/threats.tex <==
\section{Threats to Validity}
\label{sec:validity}

Since several of the inputs of our obfuscation frameworks are probabilities, 
ideally the experiment should be repetead in order to statistically rule out 
the effect of randomness on the experiment. Also, the comparably small set of 
malware samples we used for evaluation could be enlarge to obtain more 
significant results. However, as indicated in Section~\ref{sec:evaluation}, one 
experiment run takes about 27 days, which repeated several times means months. 
Nevertheless, similar results for closely related configuration settings (that 
e.g. only varied in one parameter) however indicate a rather good stability of 
the gained insights. More specifically, due to overlapping ranges of the 
probabilistic configuration parameters many similar configuration 
constellations resulted in almost identical obfuscation degrees which, despite 
us running each configuration constellation only once, gives us a good range of 
sample points of almost identical obfuscation degree.

Note, that we intentionally did not mention false positive rates of the $n$-gram approaches in our evaluation, because they are not relevant for our experiments, since we do not change or obfuscate the set of goodware during our experiments. %The false positive rates would have been interesting to show if we would have trained our classifiers with more than one instance of a malware sample, i.e. if we would have included behavioral obfuscated malware samples in the training set. However, we leave such experiments for future work.

Also, currently our experimental setting assumes the presence of a certain ground truth, i.e. the availability of a critical mass of unobfuscated malware for classifier training. If malware developers start to make more use of behavioral obfuscation mechanism the availability of such a basic training set is questionable. Using obfuscated malware for both, testing and training the classifiers, will likely diminish their effectiveness even more. For future work, we therefore also plan on investigating whether training the classifier with obfuscated instead of unobfuscated samples produces a significant impact in the results. In this particular setting it might also be interesting to investigate the effects of training the classifiers with obfuscated malware on the correct classification of goodware samples (i.e. false positives), which we currently not consider.

Having performed some initial experiments with Naive Bayes, Gaussian-kernel SVMs, and Random Forest classifiers, we can also safely say that the choice of the baseline classifier does not have a significant effect on the relative obfuscation sensitivity of the considered $n$-gram approaches.

One important aspect, which is often implicit when talking about obfuscation, is that the functionality of any obfuscated program should include the functionality of the original (non-obfuscated) program. For many software transformation engines such a compilers, this is a strict requirement. However, even very widely used compilers such as GCC or Clang have been found to contain optimizations that break the functionality of the original source code~\cite{Yang2011}. The \emph{system call reordering} transformation described in Section~\ref{sec:approach} and tested in the experiments from Section~\ref{sec:evaluation} suffers from the same issue, i.e.~it may change the functionality of malware such that it becomes ineffective. Therefore, some may argue that ineffective malware should be classified as goodware by an effective detection approach.

% The change in functionality of the obfuscated program could occur, for instance when the program expects the result from a delayed system call. We handle this by not executing the call and returning that it has been executed successfully.
% Obviously, not all delayed calls will execute without errors though, which means the application will not be able to retry at a later point in time or take action to solve the error.
% This is an obvious flaw of our tool that we do not know a solution for at this point in time.
However, we argue that in the case of obfuscating malware it is more important to be able to avoid detection even if the obfuscation engine will output some samples which are not effective. We do not yet posses statistics regarding the number of effective malware samples output by our tool however we plan to study this fact as part of future work. Note that we still consider our results valuable given the fact that checking for behavioral equality in general is not decidable and in our experiments none of the obfuscated malware samples crashed during execution.


